Adversarial Reconnaissance Mitigation and Modeling

Adversarial reconnaissance is a crucial step in sophisticated cyber-attacks as it enables threat actors to find the weakest points of otherwise well-defended systems. To thwart reconnaissance, defenders can employ cyber deception techniques, such as deploying honeypots. In recent years, researchers have made great strides in developing game-theoretic models to find optimal deception strategies. However, most of these game-theoretic models build on relatively simple models of adversarial reconnaissance -- even though reconnaissance should be a focus point as the very purpose of deception is to thwart reconnaissance. In this paper, we first discuss effective cyber reconnaissance mitigation techniques including deception strategies and beyond. Then we provide a review of the literature on deception games from the perspective of modeling adversarial reconnaissance, highlighting key aspects of reconnaissance that have not been adequately captured in prior work. We then describe a probability-theory based model of the adversaries' belief formation and illustrate using numerical examples that this model can capture key aspects of adversarial reconnaissance. We believe that our review and belief model can serve as a stepping stone for developing more realistic and practical deception games.

==> algorithms/VE.tex <==
\begin{algorithm}[!ht]
\DontPrintSemicolon
\tcc{
$\mathcal{B} \rightarrow$ a Bayesian network specifying joint distribution $Pr(\Omega_1, \Omega_1, ..., \Omega_n)$\\
$\chi \rightarrow$ a distribution over $\Omega$
}
  
  \KwInput{$\Omega \in \mathcal{E}, e, \mathcal{B}$}
  \KwOutput{$\chi$}

  $factors \leftarrow$ [] \;
  \ForEach{$var \in$ ORDER ($\mathcal{B}, VARS$)}
  {
  
  $factors \leftarrow$ [MAKE-FACTOR ($var, e$) $|\, factors$\,]\;
  \If{$var$ is a hidden variable}
    {
        $factors \leftarrow$ SUM-OUT($var, factors$)
    }
    }

   $\chi \leftarrow$ NORMALIZE(POINTWISE-PRODUCT ($factors$))
    


\caption{Variable Elimination Algorithm}
\label{algo:variable_elimination}
\end{algorithm}

==> tables/compare_p0f.tex <==
\begin{table}[!ht]
\centering
\caption{Compare Prediction with \textbf{p0f}}
\label{tab:p0f}
\begin{tabular}{|c|c|c|}
\hline
\textbf{} & \multicolumn{2}{c|}{\textbf{Prediction}} \\ \hline
\textbf{Node IP} & \textbf{Our Model} & \textbf{p0f} \\ \hline\hline
192.168.10.14 & Windows & Windows 7 or 8 \\ \hline
192.168.10.19 & Ubuntu & Linux 3.11 and newer \\ \hline
192.168.10.12 & Ubuntu & Linux 3.11 and newer \\ \hline
192.168.10.15 & Windows & Windows 7 or 8 \\ \hline
192.168.10.8 & Windows & Windows 7 or 8 \\ \hline
\end{tabular}
\end{table}

==> tables/final_notations.tex <==
\begin{table}[!ht]
    \centering
    \caption{Used Notations}
    \label{tab:final_notations}
    \begin{tabular}{|c|c|}
    \hline
    \textbf{Notations} & \textbf{Description}\\ \hline \hline
    
    \multicolumn{2}{|c|}{\textbf{Network Notations}}    \\ \hline
    $T$ & The whole Network \\\hline
    $\calW_T$ & Possible world for a network \\\hline\hline
    
    \multicolumn{2}{|c|}{\textbf{Node Notations}}    \\ \hline
      $N$ & A network node where $N \in T$ \\ \hline 
    %   $n_{\xi_i}$ & Server Node     \\ \hline
    %   $n_{c_i}$ & Client Node   \\ \hline
    %   $n_{N_i}$ & Network Device Node \\ \hline
      $A_{N}$ & Node Addresses \\ \hline
      $o_{N}$ & Node OS \\ \hline
      $S_{N}$ & Node Software Set \\ \hline
      $\calW_{N}$ & Possible world for a node \\ \hline
      \hline
      
      
    \multicolumn{2}{|c|}{\textbf{Belief Notations}}    \\ \hline
    $\beta$ & attacker's belief \\\hline
    $\beta_N$ & node belief \\\hline
    $\beta_T$ & network belief \\\hline\hline
     
     \multicolumn{2}{|c|}{\textbf{Observation Notations}}    \\ \hline
     $\Theta_{\psi,\delta,i}$ & a particular observation \\\hline
     $A_{\psi}^{\mu}$ & the source IP address \\\hline
     $A_{\psi}^\rho$ & the source port address \\\hline
     $H_{\psi,i}$ & the flow properties of $A_{\psi}$ \\\hline
     $A_{\delta}^\mu$ & the destination IP address \\\hline
     $A_{\delta}^\rho$ & the destination port address \\\hline
     $H_{\delta,i}$ & the flow properties of $A_{\delta}$ \\\hline
     $\phi_i$ & the transport layer protocol \\\hline
     $\sigma_i$ & the application layer protocol\\\hline $\Gamma_i$ & other observation information\\\hline
     $\Omega$ & Observation feature\\\hline
    %  \multicolumn{2}{|c|}{\textbf{Belief Notations}}    \\ \hline
    %   $\beta(n)$ & Attacker's Node Belief Set\\\hline
    %   $\beta_j(n)$ & An element of Node Belief Set\\\hline
    %   $\beta_f(n)$ & Belief that is fact \\\hline

    %  Set of scanned vulnerabilities & $V_{scan} $ \\\hline
    %  Set of vulnerabilities from Database & $V_{db} $ \\\hline

    \end{tabular}
    
\end{table}


==> tables/knowledge_base.tex <==
\begin{table}[!ht]
\caption{Example Knowledge Base for Particular Operating Systems (Windows/Linux)}
\label{tab:os_kb}
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{4}{|c|}{\textbf{OS Fingerprinting}} \\ \hline\hline
\multirow{2}{*}{\textbf{OS}} & \multicolumn{2}{c|}{\textbf{Features}} & \multirow{2}{*}{\textbf{Probability}} \\ \cline{2-3}
 & \textbf{TTL} & \textbf{WS} &  \\ \hline\hline
\multirow{4}{*}{Windows NT 6.x} & 120-128 & N/A & 0.24 \\ \cline{2-4} 
& N/A & 8192 & 0.24 \\ \cline{2-4} 
& 120-128 & 8192 & 0.5 \\ \cline{2-4} 
 & \multicolumn{2}{c|}{Else} & 0.02 \\ \hline
\multirow{4}{*}{Linux(kernel 2.4/ 2.6)} & 55-64 & N/A & 0.24 \\ \cline{2-4} 
& N/A & 5840 & 0.24 \\ \cline{2-4} 
& 55-64 & 5840 & 0.5 \\ \cline{2-4} 
 & \multicolumn{2}{c|}{Else} & 0.02 \\ \hline
\end{tabular}
\end{table}

\begin{table}[!ht]
\caption{Example Knowledge Base for Particular Applications (Apache/IIS)}
\label{tab:sw_kb}
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{4}{|c|}{\textbf{SW Fingerprinting}} \\ \hline\hline
\textbf{SW} & \multicolumn{2}{c|}{\textbf{Banner}} & \textbf{Probability} \\ \hline\hline
\multirow{2}{*}{Apache} & \multicolumn{2}{c|}{Apache} & 0.99 \\ \cline{2-4} 
 & \multicolumn{2}{c|}{Else} & 0.01 \\ \hline
\multirow{2}{*}{IIS} & \multicolumn{2}{c|}{Internet Information Server} & 0.99 \\ \cline{2-4} 
 & \multicolumn{2}{c|}{Else} & 0.01 \\ \hline
\end{tabular}
\end{table}

==> tables/lit_comparison.tex <==
\begin{table}[!ht]
\centering
\caption{Comparing Existing Reconnaissance Belief Update Models with Our Model}
\label{tab:comparison}
% \resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|}
\hline
\diagbox[width=12em]{Features}{Works}     &
% \begin{tabular}[c]{@{}c@{}}Siboni et\\ al., 2019 \end{tabular} &
\begin{tabular}[c]{@{}c@{}}Jajodia et\\ al., 2017\end{tabular} & \begin{tabular}[c]{@{}c@{}}Sugrim et\\ al., 2018\end{tabular} \\ \hline\hline
\begin{tabular}[c]{@{}c@{}}Configuration Consideration\\(OS, Application/Service) \end{tabular} & \checkmark & x   \\\hline
\begin{tabular}[c]{@{}c@{}}Bayesian Inference\end{tabular}  &  x &  \checkmark  \\ \hline
\begin{tabular}[c]{@{}c@{}}Reconnaissance Type\end{tabular} & \begin{tabular}[c]{@{}c@{}}Active/Passive\end{tabular} &  Active  \\ \hline
\begin{tabular}[c]{@{}c@{}}Considered Node Entity\end{tabular} & Multiple &  Single  \\ \hline
\begin{tabular}[c]{@{}c@{}}Concise Observation Model\end{tabular} & x &  x  \\ \hline
\begin{tabular}[c]{@{}c@{}}Optimized Knowledge Base\end{tabular} & x &  x   \\ \hline
\begin{tabular}[c]{@{}c@{}}Belief Update\end{tabular} & \begin{tabular}[c]{@{}c@{}}Node/Network\end{tabular} &  Network   \\ \hline
\end{tabular}
% }
\end{table}




% \begin{table}[!ht]
% \centering
% \caption{Comparing Existing Reconnaissance Belief Update Models with Our Model}
% \label{tab:comparison}
% % \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|}
% \hline
% \diagbox[width=12em]{Features}{Works}     &
% % \begin{tabular}[c]{@{}c@{}}Siboni et\\ al., 2019 \end{tabular} &
% \begin{tabular}[c]{@{}c@{}}Jajodia et\\ al., 2017\end{tabular} & \begin{tabular}[c]{@{}c@{}}Sugrim et\\ al., 2018\end{tabular} & Our Work \\ \hline\hline
% \begin{tabular}[c]{@{}c@{}}Configuration Consideration\\(OS, Application/Service) \end{tabular} & \checkmark & x  & \checkmark \\\hline
% \begin{tabular}[c]{@{}c@{}}Bayesian Inference\end{tabular}  &  x &  \checkmark & \checkmark \\ \hline
% \begin{tabular}[c]{@{}c@{}}Reconnaissance Type\end{tabular} & \begin{tabular}[c]{@{}c@{}}Active/Passive\end{tabular} &  Active &  Passive \\ \hline
% \begin{tabular}[c]{@{}c@{}}Considered Node Entity\end{tabular} & Multiple &  Single &  Multiple \\ \hline
% \begin{tabular}[c]{@{}c@{}}Concise Observation Model\end{tabular} & x &  x &  \checkmark \\ \hline
% \begin{tabular}[c]{@{}c@{}}Optimized Knowledge Base\end{tabular} & x &  x &  \checkmark  \\ \hline
% \begin{tabular}[c]{@{}c@{}}Belief Update\end{tabular} & \begin{tabular}[c]{@{}c@{}}Node/Network\end{tabular} &  Network &  \begin{tabular}[c]{@{}c@{}}Node/Network\end{tabular}  \\ \hline
% \end{tabular}
% % }
% \end{table}

==> tables/passive_recon.tex <==
\begin{table*}
\centering
\caption{Passive Reconnaissance Tools, Operations, and Collected Information}
\label{tab:passive_scan}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|}
\hline
\textbf{Reconnaissance Tools}             & \textbf{Passive Operations} & \textbf{Collected Info} \\ \hline\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Ettercap, XProbe2,\\Wireshark\end{tabular}} & Passive LAN Scan        & \begin{tabular}[c]{@{}c@{}}OS, Open Ports, Running Services,\\ IP and MAC Addresses\end{tabular}         \\ \cline{2-3} 
                          & Sniffing (IP/MAC-based) & \begin{tabular}[c]{@{}c@{}}Packet Source and Destinations,\\ Active hosts, running services\end{tabular} \\ \hline
                %   &            &                \\ \hline
\multirow{2}{*}{P0f, SinFP, Nmap} & OS Fingerprinting  &  OS Signature, OS Version \\ \cline{2-3} 
                  & Sniffing  &  \begin{tabular}[c]{@{}c@{}}open ports, running services,\\ and installed applications with version \end{tabular} \\ \hline

\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}NetworkMiner\\PacketFence, PRADS\end{tabular}}   &  OS Fingerprinting  &  OS Signature \\ \cline{2-3} 
                  & Sniffing  & \begin{tabular}[c]{@{}c@{}} Open ports, IP addresses,\\ files (e.g. image files), login credentials \end{tabular} \\ \hline
                  
\multirow{2}{*}{NetSleuth, Satori}   &  Sniffing   &  \begin{tabular}[c]{@{}c@{}}Realtime Overview of Connected hosts,\\ Open ports, IP addresses \end{tabular}\\ \cline{2-3} 
                & Device Identification  & \begin{tabular}[c]{@{}c@{}} Identify  printers, routers,\\smartphones, gaming consoles,
desktop \end{tabular}\\ \hline

\multirow{2}{*}{Cain \& Abel}   &  Sniffing   &  Routing Protocols, VOIP Conversations \\ \cline{2-3} 
                & Password Cracking  &  \begin{tabular}[c]{@{}c@{}}encrypted passwords, wireless network keys,\\ password boxes, cached passwords\end{tabular}\\ \hline

\begin{tabular}[c]{@{}c@{}}Tenable Passive\\Vulnerability Scanner \end{tabular}
                & Network Profiling  &  Topology, Installed Applications, and vulnerabilities \\ \hline

\end{tabular}
}
\end{table*}
